Sweep Complexity Revisited

We study the sweep complexity of DFA in one-way jumping mode answering several questions posed earlier. This measure is the number of times in the worst case that such machines have to return to the beginning of their input after having skipped some of the symbols. The class of languages accepted by these machines strictly includes the regular class and constant sweep complexity allows exactly the acceptance of regular languages. However, we show that there exist machines with higher than constant complexity still only accepting regular languages and that in general the sweep complexity of an automaton does not distinguish between accepting regular and non-regular languages. We establish separation results for asymptotic classes defined by this complexity measure and give a surprising exponential/logarithmic relation between factors of certain inputs which can be verified by such machines.

==> rev_Sec_append.tex <==
\begin{figure}[h]
    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three1}
        \caption{$\mathcal{B}_1$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three2}
        \caption{$\mathcal{B}_2$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three3}
        \caption{$\mathcal{B}_3$}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three4}
        \caption{$\mathcal{B}_4$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three5}
        \caption{$\mathcal{B}_5$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three6}
        \caption{$\mathcal{B}_6$}
    \end{subfigure}  

    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three7}
        \caption{$\mathcal{B}_7$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three8}
        \caption{$\mathcal{B}_8$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \input{fig/three9}
        \caption{$\mathcal{B}_9$}
    \end{subfigure}
    
    \caption{All three-state machines satisfying Lemma~\ref{nonconstantsweeps}}
    \label{fig:three}
\end{figure}

\input{rev_threestate}

\begin{figure}[h]
    \begin{subfigure}[b]{0.4\textwidth}
        \input{fig/four1}
        \caption{$\mathcal{C}_1$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \input{fig/four2}
        \caption{$\mathcal{C}_2$}
    \end{subfigure}
    
    \caption{Some four-state machines satisfying Lemma~\ref{nonconstantsweeps}}
    \label{fig:my_label}
\end{figure}
